Structured Agentic Learning for Persistent Spatial Acquisition in RDT-TAIS-Assisted Communications

Persistent TAIS operation can reduce repeated radio-information acquisition by reusing environmental knowledge across control intervals. This knowledge changes with radio-environment evolution and current communication task. This paper studies persistent spatial knowledge maintenance for TAIS control and formulates it as a sequential information-acquisition problem that maximizes effective communication performance while accounting for physical-acquisition overhead under an outage-reliability constraint. We develop structured agentic spatial intelligence (ASI), which realizes a communication-oriented agent that maintains persistent spatial knowledge, forms beliefs from radio and context observations, and adapts physical information acquisition through closed-loop interaction with the radio environment. By jointly exploiting radio-consistent context inference, temporal knowledge-sufficiency assessment, graph-structured regional reasoning, and predictive outage-risk feedback, structured ASI determines when additional acquisition is needed, where it is directed, and how much physical information is sufficient before stopping or escalating to full radio-environment reacquisition. Numerical results show that structured ASI improves the effective rate by 2.59% while reducing acquisition overhead by 25.0% at six structural changes per 100 control intervals, and achieves a 2.82% effective-rate gain with a 41.8% overhead reduction over a heterogeneous 400-interval mission.

==> sections/problem.tex <==
% ============================================================
% III. PROBLEM FORMULATION
% ============================================================
\subsection{Problem Formulation}
\label{sec:problem_formulation}

Regional information can remain useful beyond the interval of acquisition, while its physical validity evolves with the structural-change support $\mathcal D_t$ in \eqref{eq:structural_change_support} and its task relevance is determined by $\mathcal V^{\rm rel}(\chi_t)$ in \eqref{eq:task_relevant_support}.

% ============================================================
\subsubsection{Persistent Spatial Knowledge}
\label{subsec:persistent_knowledge}

The controller retains information from previous physical acquisition through a persistent spatial memory. For each region, the memory records the maintained regional state estimate, its uncertainty and age~\cite{polyzos2024bayesian,cao2025channeltwinning}. At the end of control interval $t$, this memory is represented as
\begin{equation}
    \mathcal M_t
    =
    \left\{
        \widehat{\mathbf s}_{k,t},
        \mathbf\Sigma_{k,t},
        a_{k,t}
    \right\}_{k\in\mathcal V},
    \label{eq:persistent_knowledge_state}
\end{equation}
where
$\widehat{\mathbf s}_{k,t}\in\mathbb R^{d_s}$ is the maintained
estimate of the persistent regional state $\mathbf s_{k,t}$,
$\mathbf\Sigma_{k,t}\in\mathbb R^{d_s\times d_s}$ with
$\mathbf\Sigma_{k,t}\succeq\mathbf 0$ quantifies the associated uncertainty,
and $a_{k,t}$ is the knowledge age.
The age records the number of control intervals elapsed since the latest
regional or full reacquisition of region $k$.
An initial memory state $\mathcal M_0$ is available before online operation.

At the beginning of interval $t$, the controller combines the retained memory
with the current routine observations and the preceding operating condition.
The resulting pre-acquisition information state is given by
\begin{equation}
    \mathcal I_t^{-}
    =
    \left\{
        \mathcal M_{t-1},
        \mathbf r_t,
        \widetilde{\chi}_t,
        \boldsymbol{\phi}_{t-1},
        R_{t-1}
    \right\},
    \label{eq:pre_acquisition_information}
\end{equation}
where $R_{t-1}$ is the payload-transmission rate achieved in the preceding
control interval.
The corresponding initial operating quantities are available at $t=1$.

% ============================================================
\subsubsection{Acquisition--Service Tradeoff}
\label{subsec:acquisition_service_tradeoff}


We characterize the communication service and reliability under the
acquisition overhead $N^{\rm acq}$ through the payload rate, effective rate,
and outage probability.
With maximal ratio combining (MRC) at the BS, the payload-transmission rate during
interval $t$ is given by~\cite{liu2026taismu}
\begin{equation}
    R_t
    =
    \log_2
    \Big(
        1+
        \frac{
            P_{\rm u}
            \left\|
                \mathbf F_t
                \mathbf\Phi_t
                \mathbf h_t
            \right\|^2
        }{
            \sigma_0^2
        }
    \Big),
    \label{eq:instantaneous_rate}
\end{equation}


The net communication service is quantified by the acquisition-adjusted
effective rate, given by
\begin{equation}
    R_{\rm eff}
    =
    \frac{
        N_{\rm sym}        
    }{
        T N_{\rm sym}
        +
        N_{\rm acq}
    } \displaystyle\sum_{t=1}^{T} R_t
    \label{eq:effective_rate}
\end{equation}
where $N_{\rm sym}$ is the number of OFDM symbols allocated to payload
transmission in each control interval.
The numerator is the accumulated payload service, while the
denominator accounts for the radio resources occupied by payload transmission
and dedicated physical acquisition.
% Updated environmental information can increase $R_t$ through the resulting
% TAIS configuration, while selective reuse controls $N_{\rm acq}$.

Communication reliability is characterized through the horizon-averaged
outage probability, given by
\begin{equation}
    P_{\rm out}
    =
    \frac{1}{T}
    \sum_{t=1}^{T}
    \Pr
    \left(
        R_t<R_{\rm th}
    \right),
    \label{eq:outage_probability}
\end{equation}
where $R_{\rm th}$ is the prescribed payload-rate target.


% Together, $R_{\rm eff}$ in \eqref{eq:effective_rate} and $P_{\rm out}$ in
% \eqref{eq:outage_probability} quantify the communication service and
% reliability achieved under the acquisition overhead $N_{\rm acq}$.
% They provide the communication objective and reliability criterion governing
% the persistent spatial memory policy.

% ============================================================
\subsubsection{Sequential Verification--Reacquisition Policy}
\label{subsec:sequential_control_problem}

The causal acquisition policy is represented by
$\pi_{\rm acq}=(\pi_{\rm loc},\pi_{\rm reacq},\pi_{\rm full})$.
Starting from $\mathcal I_t^{-}$ in
\eqref{eq:pre_acquisition_information}, let
$\mathcal I_{t,\ell-1}$ denote the controller information after
$\ell-1$ completed regional verification steps, with
$\mathcal I_{t,0}=\mathcal I_t^{-}$.
At regional verification step $\ell$, the regional selection policy is given
by
\begin{equation}
    k_{t,\ell}
    =
    \pi_{\rm loc}
    \left(
        \mathcal I_{t,\ell-1}
    \right),
    \qquad
    k_{t,\ell}
    \in
    \mathcal V\cup\{\mathtt{stop}\},
    \label{eq:regional_selection}
\end{equation}
where a selected region $k_{t,\ell}\in\mathcal V$ produces the verification
observation
$\mathbf y_{k_{t,\ell},t}^{\rm ver}$ through
\eqref{eq:regional_verification_observation}.
$\pi_{\rm reacq}$ maps
$\mathcal I_{t,\ell-1}$ and
$\mathbf y_{k_{t,\ell},t}^{\rm ver}$ to the regional reacquisition decision
$b_{t,\ell}^{\rm reacq}\in\{0,1\}$.
$b_{t,\ell}^{\rm reacq}=1$ activates the regional reacquisition in
\eqref{eq:regional_reacquisition_observation}.
The verification observation and any regional reacquisition are incorporated
into $\mathcal I_{t,\ell}$ before the subsequent regional decision~\cite{Zhang2025RISActiveCodebook,Han2025RISActiveTracking}.

After $L_t$ completed regional verification steps, the terminal regional
information is
$\mathcal I_t^{\rm loc}\triangleq\mathcal I_{t,L_t}$.
The component $\pi_{\rm full}$ maps $\mathcal I_t^{\rm loc}$ to the
full-reacquisition decision $b_t^{\rm full}\in\{0,1\}$.
The resulting acquisition stage produces the post-acquisition information
state $\mathcal I_t^{+}$ and updates the persistent memory to~$\mathcal M_t$.

The post-acquisition information state is converted into the TAIS configuration
for payload transmission through the knowledge-conditioned TAIS controller,
as given by
\begin{equation}
    \boldsymbol{\phi}_t
    =
    \pi_{\rm TAIS}
    \left(
        \mathcal I_t^{+}
    \right),
    \qquad
    \boldsymbol{\phi}_t\in\mathcal A,
    \label{eq:tais_policy}
\end{equation}
where $\pi_{\rm TAIS}$ denotes the knowledge-conditioned TAIS controller that maps the acquired environmental information to the
payload configuration across all acquisition policies and remains
fixed throughout the acquisition-policy design.

The controller seeks a causal acquisition policy that maximizes the
acquisition-adjusted communication performance under the prescribed
reliability requirement~\cite{Moss2024ConstrainedZero,
      ReyhanColeri2025SafeDRL,
      ZhaoMao2025TwoTimescale}.
The persistent spatial knowledge-maintenance problem is
cast as
\begin{subequations}
\label{prob:joint_problem}
\begin{align}
    \text{\rm \textbf{P1:}}\qquad
    \underset{
        \pi_{\rm acq}\in\Pi_{\rm acq}^{\rm causal}
    }{\operatorname{max}}
    \quad&
    \mathbb E_{\pi_{\rm acq}}
    \left[
        R_{\rm eff}
    \right]
    \label{prob:joint_problem_obj}
    \\
    \mathrm{s.t.}\quad&
    P_{\rm out}
    \left(
        \pi_{\rm acq}
    \right)
    \leq
    \epsilon,
    \label{prob:joint_problem_outage}
\end{align}
\end{subequations}
where $\Pi_{\rm acq}^{\rm causal}$ denotes the set of acquisition policies
using the controller information available at each decision step and
following the above verification--reacquisition structure, and $\epsilon$
denotes the prescribed horizon-level outage tolerance.


